Scopeformer: n-CNN-ViT Hybrid Model for Intracranial Hemorrhage Classification

We propose a feature generator backbone composed of an ensemble of convolutional neuralnetworks (CNNs) to improve the recently emerging Vision Transformer (ViT) models. We tackled the RSNA intracranial hemorrhage classification problem, i.e., identifying various hemorrhage types from computed tomography (CT) slices. We show that by gradually stacking several feature maps extracted using multiple Xception CNNs, we can develop a feature-rich input for the ViT model. Our approach allowed the ViT model to pay attention to relevant features at multiple levels. Moreover, pretraining the n CNNs using various paradigms leads to a diverse feature set and further improves the performance of the proposed n-CNN-ViT. We achieved a test accuracy of 98.04% with a weighted logarithmic loss value of 0.0708. The proposed architecture is modular and scalable in both the number of CNNs used for feature extraction and the size of the ViT.

==> bibliography.tex <==
@misc{vit-paper,
      title={An Image is Worth 16x16 Words: Transformers for Image Recognition at Scale}, 
      author={Alexey Dosovitskiy and Lucas Beyer and Alexander Kolesnikov and Dirk Weissenborn and Xiaohua Zhai and Thomas Unterthiner and Mostafa Dehghani and Matthias Minderer and Georg Heigold and Sylvain Gelly and Jakob Uszkoreit and Neil Houlsby},
      year={2020},
      eprint={2010.11929},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@misc{RSNA,
      title={ Construction of a machine learning dataset through collaboration: the RSNA 2019 brain CT hemorrhage challenge. Radiology}, 
      author={Flanders AE, Prevedello LM, Shih G et al (2020)},
      year = {2019}
}

@misc{loss,
      title={ Accurate and Efficient Intracranial Hemorrhage Detection and Subtype Classification in 3D CT Scans with Convolutional and Long Short-Term Memory Neural Networks. Sensors.}, 
      author={Burduja M, Ionescu RT, Verga N.},
      year = {2020}
}


@misc{gan-paper,
      title={Generative Adversarial Networks}, 
      author={Ian J. Goodfellow and Jean Pouget-Abadie and Mehdi Mirza and Bing Xu and David Warde-Farley and Sherjil Ozair and Aaron Courville and Yoshua Bengio},
      year={2014},
      eprint={1406.2661},
      archivePrefix={arXiv},
      primaryClass={stat.ML}
}

@inproceedings{xception-paper,
  title={Xception: Deep Learning with Depthwise Separable Convolutions},
  author={Chollet, Francois},
  booktitle={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={1800--1807},
  year={2017},
  organization={IEEE Computer Society}
}

@article{hu-window-radio,
  title={Acute stroke: improved nonenhanced CT detection—benefits of soft-copy interpretation by using variable window width and center level settings},
  author={Lev, Michael H and Farkas, Jeffrey and Gemmete, Joseph J and Hossain, Syeda T and Hunter, George J and Koroshetz, Walter J and Gonzalez, R Gilberto},
  journal={Radiology},
  volume={213},
  number={1},
  pages={150--155},
  year={1999},
  publisher={Radiological Society of North America}
}

